Decomposing a Recurrent Neural Network into Modules for Enabling Reusability and Replacement

Can we take a recurrent neural network (RNN) trained to translate between languages and augment it to support a new natural language without retraining the model from scratch? Can we fix the faulty behavior of the RNN by replacing portions associated with the faulty behavior? Recent works on decomposing a fully connected neural network (FCNN) and convolutional neural network (CNN) into modules have shown the value of engineering deep models in this manner, which is standard in traditional SE but foreign for deep learning models. However, prior works focus on the image-based multiclass classification problems and cannot be applied to RNN due to (a) different layer structures, (b) loop structures, (c) different types of input-output architectures, and (d) usage of both nonlinear and logistic activation functions. In this work, we propose the first approach to decompose an RNN into modules. We study different types of RNNs, i.e., Vanilla, LSTM, and GRU. Further, we show how such RNN modules can be reused and replaced in various scenarios. We evaluate our approach against 5 canonical datasets (i.e., Math QA, Brown Corpus, Wiki-toxicity, Clinc OOS, and Tatoeba) and 4 model variants for each dataset. We found that decomposing a trained model has a small cost (Accuracy: -0.6%, BLEU score: +0.10%). Also, the decomposed modules can be reused and replaced without needing to retrain.

==> replaceres.tex <==
 \begin{figure*}[htp]
        \centering
            \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/intra-1-1.pdf}} 
            \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/intra-1-M.pdf}}
            \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/intra-M-1.pdf}}
            \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/intra-M-M.pdf}}
            \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/inter--1-1.pdf}}
            \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/inter-M-M.pdf}}
        \caption{\change{Results for Replace Experiments (a) One-to-one Intra replace (b) One-to-many Intra replace (c) Many-to-one Intra replace (d) Many-to-many Intra replace (e) OneOne-OneMany Inter replace (f) ManyOne-ManyMany Inter replace}}
        \label{fig: replace}
        \end{figure*}
        
% \begin{figure*}[htp]
%         \centering
%             \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/RQ311-cropped.pdf}} 
%             \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/RQ31M-cropped.pdf}}
%             \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/RQ3M1-cropped.pdf}}
            
%             \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/RQ3MM-cropped.pdf}}
%             \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/RQ3inter11-cropped.pdf}}
%             \subfigure[]{\includegraphics[width=.25\textwidth]{replace-charts/RQ3interMM-cropped.pdf}}
%         \caption{\change{Results for Replace Experiments (a) One-to-one Intra replace (b) One-to-many Intra replace (c) Many-to-one Intra replace (d) Many-to-many Intra replace (e) OneOne-OneMany Inter replace (f) ManyOne-ManyMany Inter replace}}
%         \label{fig: replace}
%         \end{figure*}

==> reuseres.tex <==
 \begin{figure*}[htp]
        \centering
            \subfigure[]{\includegraphics[width=.23\textwidth]{reuse-charts/RQ211-cropped.pdf}} 
            \subfigure[]{\includegraphics[width=.23\textwidth]{reuse-charts/RQ21M-cropped.pdf}}
            \subfigure[]{\includegraphics[width=.23\textwidth]{reuse-charts/RQ2M1-cropped.pdf}}
            \subfigure[]{\includegraphics[width=.23\textwidth]{reuse-charts/RQ2MM-cropped.pdf}}\\
            \subfigure[]{\includegraphics[width=.25\textwidth]{reuse-charts/RQ2inter11-cropped.pdf}}
            \subfigure[]{\includegraphics[width=.25\textwidth]{reuse-charts/RQ2interMM-cropped.pdf}}
            \subfigure[]{\includegraphics[width=.25\textwidth]{reuse-charts/RQ2LM-cropped.pdf}}
        \caption{\change{}}
        \label{fig: reuse}
        \end{figure*}

==> rq1res.tex <==

 
 \begin{figure*}[htp]
        \centering
            \subfigure[]{\includegraphics[width=.23\textwidth]{rq1graphs/RQ111-cropped.pdf}} 
            \subfigure[]{\includegraphics[width=.23\textwidth]{rq1graphs/RQ1M1-cropped.pdf}}
            \subfigure[]{\includegraphics[width=.23\textwidth]{rq1graphs/RQ11M-cropped.pdf}}
            \subfigure[]{\includegraphics[width=.23\textwidth]{rq1graphs/RQ1MM-cropped.pdf}}\\
            \subfigure[]{\includegraphics[width=.23\textwidth]{rq1graphs/ENFR-cropped.pdf}}
            \subfigure[]{\includegraphics[width=.23\textwidth]{rq1graphs/ENDE-cropped.pdf}}
            \subfigure[]{\includegraphics[width=.23\textwidth]{rq1graphs/ENIT-cropped.pdf}}
        \caption{\change{}}
        \label{fig: replace}
        \end{figure*}

==> rq1tb.tex <==
% Table generated by Excel2LaTeX from sheet 'RQ1'
\begin{table*}[htbp]
  \centering
  \footnotesize
  \caption{Cost of Decomposing RNN into Modules.}
  \vspace{1pt}
  \setlength\tabcolsep{1pt}
    \begin{tabular}{|c|c|c|r|r|r|r|r|r|r|r|r|r|r|}
    \hline
    \multirow{2}{*}{\textbf{Model Type}} & \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Monolithic Model Accuracy}}} & \multicolumn{4}{c|}{\textbf{Rolled}} & \multicolumn{4}{c|}{\textbf{Unrolled}} \\
\cline{7-14}          &       &       & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{\textbf{Composed Model Accuracy}} & \multicolumn{1}{c|}{\textbf{JI}} & \multicolumn{3}{c|}{\textbf{Composed Model Accuracy}} & \multicolumn{1}{c|}{\textbf{JI}} \\
    \hline
    \hline
    \multirow{4}{*}{One-to-One} & \multirow{4}{*}{Math QA} & RNN-1 & \multicolumn{3}{r|}{97.42\%} & \multicolumn{3}{r|}{97.12\%} & 0.50   & \multicolumn{3}{r|}{\cellcolor[rgb]{ 0,  0,  0}\textbf{Domain 6}} & \cellcolor[rgb]{ 0,  0,  0}\textbf{Domain 6} \\
\cline{3-14}          &       & RNN-2 & \multicolumn{3}{r|}{96.72\%} & \multicolumn{3}{r|}{96.05\%} & 0.55  & \multicolumn{3}{r|}{\cellcolor[rgb]{ 0,  0,  0}\textbf{Domain 6}} & \cellcolor[rgb]{ 0,  0,  0}\textbf{Domain 6} \\
\cline{3-14}          &       & RNN-3 & \multicolumn{3}{r|}{95.85\%} & \multicolumn{3}{r|}{95.21\%} & 0.57  & \multicolumn{3}{r|}{\cellcolor[rgb]{ 0,  0,  0}\textbf{Domain 6}} & \cellcolor[rgb]{ 0,  0,  0}\textbf{Domain 6} \\
\cline{3-14}          &       & RNN-4 & \multicolumn{3}{r|}{95.98\%} & \multicolumn{3}{r|}{94.98\%} & 0.69  & \multicolumn{3}{r|}{\cellcolor[rgb]{ 0,  0,  0}\textbf{Domain 6}} & \cellcolor[rgb]{ 0,  0,  0}\textbf{Domain 6} \\
    \hline
    \multirow{4}{*}{Many-to-One} & \multirow{4}{*}{Clinc OOS} & RNN-1 & \multicolumn{3}{r|}{93.42\%} & \multicolumn{3}{r|}{91.84\%} & 0.71  & \multicolumn{3}{r|}{93.35\%} & 0.72 \\
\cline{3-14}          &       & RNN-2 & \multicolumn{3}{r|}{94.02\%} & \multicolumn{3}{r|}{88.51\%} & 0.81  & \multicolumn{3}{r|}{92.64\%} & 0.81 \\
\cline{3-14}          &       & RNN-3 & \multicolumn{3}{r|}{93.31\%} & \multicolumn{3}{r|}{91.04\%} & 0.84  & \multicolumn{3}{r|}{92.44\%} & 0.89 \\
\cline{3-14}          &       & RNN-4 & \multicolumn{3}{r|}{93.13\%} & \multicolumn{3}{r|}{90.73\%} & 0.88  & \multicolumn{3}{r|}{93.02\%} & 0.89 \\
    \hline
    \multirow{4}{*}{One-to-Many} & \multirow{4}{*}{Toxic Comment} & RNN-1 & \multicolumn{3}{r|}{96.40\%} & \multicolumn{3}{r|}{81.19\%} & 0.67  & \multicolumn{3}{r|}{95.43\%} & 0.71 \\
\cline{3-14}          &       & RNN-2 & \multicolumn{3}{r|}{96.15\%} & \multicolumn{3}{r|}{81.19\%} & 0.80  & \multicolumn{3}{r|}{94.67\%} & 0.83 \\
\cline{3-14}          &       & RNN-3 & \multicolumn{3}{r|}{96.33\%} & \multicolumn{3}{r|}{81.19\%} & 0.83  & \multicolumn{3}{r|}{95.97\%} & 0.84 \\
\cline{3-14}          &       & RNN-4 & \multicolumn{3}{r|}{96.46\%} & \multicolumn{3}{r|}{81.19\%} & 0.82   & \multicolumn{3}{r|}{93.68\%} & 0.83 \\
    \hline
    \multicolumn{1}{|c|}{\multirow{4}{*}{\makecell[c]{Many-to-Many\\ (Traditional)}}} & \multirow{4}{*}{Brown Corpus} & RNN-1 & \multicolumn{3}{r|}{96.13\%} & \multicolumn{3}{r|}{16.25\%} & 0.67  & \multicolumn{3}{r|}{93.68\%} & 0.67 \\
\cline{3-14}          &       & RNN-2 & \multicolumn{3}{r|}{96.18\%} & \multicolumn{3}{r|}{16.25\%} & 0.74  & \multicolumn{3}{r|}{94.54\%} & 0.74 \\
\cline{3-14}          &       & RNN-3 & \multicolumn{3}{r|}{95.93\%} & \multicolumn{3}{r|}{16.25\%} & 0.78  & \multicolumn{3}{r|}{93.03\%} & 0.78 \\
\cline{3-14}          &       & RNN-4 & \multicolumn{3}{r|}{95.93\%} & \multicolumn{3}{r|}{16.25\%} & 0.82  & \multicolumn{3}{r|}{92.56\%} & 0.83 \\
    \hline
    \multicolumn{1}{|c|}{\multirow{6}{*}{\makecell[c]{Many-to-Many\\ (Encoder-Decoder)}}} & \multirow{6}{*}{Tatoeba} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{BLEU}} & \multicolumn{3}{c|}{\textbf{BLEU}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{JI}}} & \multicolumn{3}{c|}{\textbf{BLEU}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{JI}}} \\
\cline{4-9}\cline{11-13}          &       &       & \multicolumn{1}{c|}{\textbf{EN-FR}} & \multicolumn{1}{c|}{\textbf{EN-DE}} & \multicolumn{1}{c|}{\textbf{EN-IT}} & \multicolumn{1}{c|}{\textbf{EN-FR}} & \multicolumn{1}{c|}{\textbf{EN-DE}} & \multicolumn{1}{c|}{\textbf{EN-IT}} &       & \multicolumn{1}{c|}{\textbf{EN-FR}} & \multicolumn{1}{c|}{\textbf{EN-DE}} & \multicolumn{1}{c|}{\textbf{EN-IT}} &  \\
\cline{3-14}          &       & RNN-1 &    25.92\%   &  29.54\%      &  27.82\%     &  \cellcolor[rgb]{ .776,  .878,  .706}\textbf{26.05\%}     &   29.52\%    &  27.25\%    & 0.70      &  25.67\%     &   28.69\%    &  \cellcolor[rgb]{ .776,  .878,  .706}\textbf{28.58\%}     & 0.69 \\
\cline{3-14}          &       & RNN-2 &   24.82\%      &   26.07\%    &  24.32\%   & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{24.98\%} &   25.59\%   &    22.72\%   &     0.71 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{25.07\%}     &   25.81\%     &  23.80\%     & 0.70 \\
\cline{3-14}          &       & RNN-3 &    26.57\%     &  29.67\%     &  24.81\%   & 25.89\% &  29.11\%    &   \cellcolor[rgb]{ .776,  .878,  .706}\textbf{27.19\%}    &  0.71    &  26.19\%    &    26.67\%    &   \cellcolor[rgb]{ .776,  .878,  .706}\textbf{28.40\%}   & 0.70 \\
\cline{3-14}          &       & RNN-4 &  26.87\%       &   29.39\%    &  26.27\%   & 25.83\% &  29.11\%    & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{28.78\%}      & 0.70     & 24.41\%     &  29.05\%      &   25.79\%    & 0.69 \\
% \cline{3-14}          &       & RNN-4 &         &       &     &  &      &       &      &      &        &       &  \\

    \hline
    \end{tabular}%
  \label{tb:RQ1}%
\end{table*}%




==> rq3Inter.tex <==
% Table generated by Excel2LaTeX from sheet 'Reuse-Inter1 1-1 N'
\begin{table*}[htbp]
 \centering
 \footnotesize
 \vspace{-1pt}
   \setlength\tabcolsep{0pt}
  \caption{One-to-One and One-to-Many Inter Replacement. MA, TMA: Decomposed, Trained Model Accuracy. }
  \vspace{1pt}
    \begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline  \multicolumn{1}{|l|}{\textbf{Toxic Comment}} & \multicolumn{2}{c|}{\textbf{Neutral}} & \multicolumn{2}{c|}{\textbf{Toxic}} & \multicolumn{2}{c|}{\textbf{Severe Toxic}} & \multicolumn{2}{c|}{\textbf{Obscene}} & \multicolumn{2}{c|}{\textbf{Threat}} & \multicolumn{2}{c|}{\textbf{Insult}} & \multicolumn{2}{c|}{\textbf{Identity Threat}} \\
\hline    \multicolumn{1}{|l|}{\textbf{Math QA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} \\
    \hline
    \hline
    \textbf{Gain} & 64.5\% & 80.6\% & 75.6\% & 89.8\% & 92.7\% & 81.4\% & 68.7\% & 86.9\% & 89.8\% & 85.3\% & 72.3\% & 84.7\% & 83.9\% & 81.6\% \\
    \hline
    \textbf{General} & 77.3\% & 90.3\% & 81.9\% & 88.2\% & \textbf{93.6\%} & \textbf{87.4\%} & 76.9\% & 89.1\% & \textbf{90.0\%} & \textbf{87.2\%} & 77.9\% & 89.1\% & 84.0\% & 85.7\% \\
    \hline
    \textbf{Geometry} & 62.3\% & 85.9\% & 73.3\% & 86.1\% & \textbf{93.0\%} & \textbf{79.6\%} & 68.2\% & 82.5\% & \textbf{90.6\% }& \textbf{78.9\%} & 72.3\% & 81.8\% & \textbf{84.8\%} & \textbf{82.4\%} \\
    \hline
    \textbf{Other} & 66.1\% & 90.5\% & 73.1\% & 79.4\% & \textbf{93.7\%} & \textbf{78.1\%} & 71.5\% & 78.4\% & \textbf{91.9\%} & \textbf{81.1\%} & 75.6\% & 84.5\% & \textbf{86.6\%} & \textbf{82.6\%} \\
    \hline
    \textbf{Physics} & 65.9\% & 78.0\% & 75.2\% & 82.9\% & \textbf{92.3\%} & \textbf{82.5\%} & 68.0\% & 83.1\% & \textbf{89.4\%} & \textbf{77.8\%} & 72.2\% & 84.6\% & \textbf{83.1\%} & \textbf{81.7\%} \\
    \hline
    \textbf{Probability} & 62.5\% & 93.1\% & 72.1\% & 89.9\% & \textbf{92.9\%} & \textbf{90.8\%} & 68.5\% & 91.0\% & \textbf{90.7\%} & \textbf{80.5\%} & 72.9\% & 90.8\% & 85.2\% & 89.5\% \\
    \hline
    \end{tabular}%
  \label{tb:rq3interone}\\
  \vspace{1pt}
  MA: Decomposed Module Accuracy, TMA: Trained Model Accuracy.
\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Reuse-InterN 1-N N'
\begin{table*}[htbp]
 \footnotesize
 \vspace{-1pt}
   \setlength\tabcolsep{0pt}
  \caption{Many-to-One and Many-to-Many Inter Replacement. All results are in \%.}
  \vspace{1pt}
    \begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
    \hline
    \textbf{Brown Corpus} & \multicolumn{2}{c|}{\textbf{Verb}} & \multicolumn{2}{c|}{\textbf{Noun}} & \multicolumn{2}{c|}{\textbf{Pronoun}} & \multicolumn{2}{c|}{\textbf{Adjective}} & \multicolumn{2}{c|}{\textbf{Adverb}} & \multicolumn{2}{c|}{\textbf{Adposition}} & \multicolumn{2}{c|}{\textbf{Conjunction}} & \multicolumn{2}{c|}{\textbf{Determiners}} & \multicolumn{2}{c|}{\textbf{Numbers}} & \multicolumn{2}{c|}{\textbf{Particles}} & \multicolumn{2}{c|}{\textbf{Other}} & \multicolumn{2}{c|}{\textbf{Punctuation}} \\
    \hline
    \textbf{Clinc OOS} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{MA}} & \multicolumn{1}{c|}{\textbf{TMA}} \\
    \hline
    \hline
\textbf{Work} & 97.8 & 99.4 & 98.2 & 99.2 & \textbf{99.6} & \textbf{99.6} & 98.3 & 99.6 & 97.0 & 99.5 & 98.1 & 99.3 & 97.4 & 99.5 & 96.2 & 99.6 & 98.3 & 99.9 & 95.8 & 99.5 & 97.3 & 99.7 & 94.6 & 98.5 \\
\hline
\textbf{Banking} & 99.2 & 99.7 & 99.6 & 99.8 & \textbf{99.9} & \textbf{99.7} & 99.6 & 99.8 & 98.3 & 99.8 & 99.5 & 99.7 & 99.3 & 99.8 & 98.6 & 99.5 & 99.7 & 100.0 & 99.2 & 99.6 & 99.4 & 99.8 & \textbf{99.3} & \textbf{98.3} \\
\hline
\textbf{Meta} & 96.9 & 99.3 & 96.9 & 99.6 & 99.3 & 99.7 & 96.8 & 99.5 & 96.8 & 99.4 & 95.9 & 99.4 & 96.9 & 99.5 & 94.5 & 99.7 & 96.6 & 99.9 & 96.4 & 99.6 & 91.7 & 99.2 & 82.6 & 96.3 \\
\hline
\textbf{Travel} & 96.9 & 99.2 & 97.3 & 99.2 & 99.4 & 99.6 & 97.1 & 99.3 & 96.4 & 99.5 & 96.5 & 99.2 & 96.9 & 99.7 & 94.3 & 99.5 & 97.1 & 99.9 & 94.5 & 99.2 & 95.1 & 99.6 & 87.6 & 97.0 \\
\hline
\textbf{Dining} & 97.2 & 99.3 & 97.5 & 99.4 & 99.6 & 99.7 & 97.7 & 99.4 & 96.6 & 99.5 & 97.5 & 99.7 & 97.7 & 99.5 & 95.1 & 99.5 & 98.1 & 99.7 & 97.0 & 99.0 & 96.7 & 99.3 & 93.5 & 98.9 \\
\hline
\textbf{Auto} & 97.2 & 99.3 & 97.4 & 99.3 & 99.2 & 99.3 & 97.3 & 98.6 & 96.9 & 99.5 & 97.0 & 98.8 & 97.3 & 99.3 & 95.1 & 99.3 & 96.8 & 97.7 & 96.1 & 99.5 & 93.3 & 99.3 & 83.0 & 98.5 \\
\hline
\textbf{Utility} & 96.6 & 98.2 & 96.3 & 99.3 & 99.0 & 99.5 & 95.0 & 99.3 & 96.6 & 99.6 & 94.6 & 99.4 & 92.4 & 99.7 & 93.9 & 99.8 & 92.7 & 99.7 & 90.8 & 99.6 & 90.8 & 99.3 & 80.0 & 98.7 \\
\hline
\textbf{Credit Card} & 96.9 & 98.8 & 96.9 & 99.6 & 99.2 & 99.8 & 96.6 & 99.5 & 96.5 & 99.6 & 95.5 & 99.4 & 96.6 & 99.7 & 94.0 & 99.5 & 96.0 & 99.8 & 95.7 & 99.5 & 91.1 & 99.7 & 79.3 & 98.7 \\
\hline
\textbf{Home} & 97.0 & 98.4 & 97.0 & 99.2 & 98.3 & 99.7 & 96.9 & 99.4 & 96.6 & 99.7 & 96.3 & 99.3 & 97.1 & 99.6 & 93.8 & 99.7 & 95.3 & 99.5 & 96.3 & 99.7 & 94.1 & 99.7 & 79.4 & 99.1 \\
\hline
\textbf{Small Talk} & 96.9 & 97.8 & 96.9 & 99.3 & 99.2 & 99.5 & 96.5 & 98.9 & 97.0 & 99.4 & 95.7 & 98.8 & 94.8 & 99.8 & 95.1 & 99.1 & 95.2 & 99.7 & 91.8 & 99.8 & 95.4 & 99.2 & 87.6 & 97.8 \\
    \hline
    \end{tabular}%
  \label{tb:rq3intermany}\\
%  MA: Decomposed Module Accuracy, TMA: Trained Model Accuracy.
\end{table*}%




==> rq3Intra.tex <==
% Table generated by Excel2LaTeX from sheet 'RQ3-Intra'
\begin{table*}[htbp]
  \centering
    \footnotesize
   \setlength\tabcolsep{0pt}
   
  \caption{Intra Dataset-Model Type Replacement.}
  \vspace{1pt}
    \begin{tabular}{|l|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{\textbf{Model Type}} & \multicolumn{1}{c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{TMA}} & \multicolumn{1}{c|}{\textbf{Prior MA}} & \multicolumn{1}{c|}{\textbf{RM0}} & \multicolumn{1}{c|}{\textbf{RM1}} & \multicolumn{1}{c|}{\textbf{RM2}} & \multicolumn{1}{c|}{\textbf{RM3}} & \multicolumn{1}{c|}{\textbf{RM4}} & \multicolumn{1}{c|}{\textbf{RM5}} & \multicolumn{1}{c|}{\textbf{RM6}} & \multicolumn{1}{c|}{\textbf{RM7}} & \multicolumn{1}{c|}{\textbf{RM8}} & \multicolumn{1}{c|}{\textbf{RM9}} & \multicolumn{1}{c|}{\textbf{RM10}} & \multicolumn{1}{c|}{\textbf{RM11}} \\
    \hline
    \hline
    One-to-One & Math QA &   96.62  &   95.08    &  95.51     &    94.91   &   96.25    &   94.04    &   95.11    &  95.98     &  \cellcolor[rgb]{ 0,  0,  0}     & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} \\
    \hline
    Many-to-One & Clinc OOS &  93.31     &  92.44     &   89.04    &  83.8     &   91.73    &   91.91    &   92.42    &   91.95    &  91.45     &   90.47    &  92.36     &   90.38    & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} \\
    \hline
    One-to-Many & Toxic Comment &   96.46    &   93.68  &   96.12    &   91.61    &    93.67   &    93.66   &   93.68    &  93.65     & 93.65 & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0}\\
    \hline
    Many-to-Many (Traditional) & Brown Corpus &  95.93     &    92.56   &  84.77     &  92.04     &   89.54    &   90.46    &  91.64     &  91.17  &91.17   &  92.32     &    92.43   &  91.89     &  92.50     &  92.48  \\
    \hline
    Many-to-Many (Encoder-Decoder) & Tatoeba &   25.07    & 24.89      &  \textbf{25.09}     &    \textbf{25.85}   &   \textbf{26.49}    & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} & \cellcolor[rgb]{ 0,  0,  0} \\
    \hline
    \end{tabular}%
  \label{tb:rq3Intra}\\
  \vspace{1pt}
  TMA: Trained Model Accuracy. Prior MA: Composed Accuracy of the Decomposed Modules before Replacement. RM\{\textbf{X}\}: Replace the Module with Index \textbf{X}.
\end{table*}%

